On CAD Informed Adaptive Robotic Assembly

We introduce a robotic assembly system that streamlines the design-to-make workflow for going from a CAD model of a product assembly to a fully programmed and adaptive assembly process. Our system captures (in the CAD tool) the intent of the assembly process for a specific robotic workcell and generates a recipe of task-level instructions. By integrating visual sensing with deep-learned perception models, the robots infer the necessary actions to assemble the design from the generated recipe. The perception models are trained directly from simulation, allowing the system to identify various parts based on CAD information. We demonstrate the system with a workcell of two robots to assemble interlocking 3D part designs. We first build and tune the assembly process in simulation, verifying the generated recipe. Finally, the real robotic workcell assembles the design using the same behavior.

==> related_work.tex <==
L. H. De Mello and A. C. Sanderson, “A correct and complete algorithm for the generation of mechanical assembly sequences,” IEEE transactions on Robotics and Automation, vol. 7, no. 2, pp. 228–240, 1991.

D. Halperin, J.-C. Latombe, and R. H. Wilson, “A general framework for assembly planning: The motion space approach,” Algorithmica, vol. 26, no. 3-4, pp. 577–601, 2000.

R. A. Knepper, T. Layton, J. Romanishin, and D. Rus, “Ikeabot: An autonomous multi-robot coordinated furniture assembly system,” in Robotics and Automation (ICRA), 2013 IEEE International Conference
on. IEEE, 2013, pp. 855–862.

 F. Lange, M. Suppa, and G. Hirzinger, “Control with a compliant force-torque sensor,” in Robotics; Proceedings of ROBOTIK 2012; 7th German Conference on. VDE, 2012, pp. 1–6.
 
[34] F. Lange, W. Bertleff, and M. Suppa, “Force and trajectory control of industrial robots in stiff contact,” in Robotics and Automation (ICRA), 2013IEEEInternationalConferenceon. IEEE,2013,pp.2927–2934.

H.Lasi,P.Fettke,H.-G.Kemper,T.Feld,andM.Hoffmann,“Industry 4.0,” Business & Information Systems Engineering, vol. 6, no. 4, pp. 239–242, 2014.

L. Durkop, L. Wisniewski, S. Heymann, B. Lucke, and J. Jasperneite, “Analyzing the engineering effort for the commissioning of industrial automation systems,” in  2105 IEEE 20th Conference on Emerging Technologies & Factory Automation, 2015

F. Thomas and C. Torras. Inferring feasible assemblies from spatial constraints. IEEE Transactions on Robotics and Automation, 8(2):228–239, 1992.

A. P. Ambler and R. J. Popplestone. Inferring the positions of bodies from specified spatial relationships. Artificial Intel- ligence, 6:157–174, 1975.

J. Latombe R.H. Wilson. Geometric reasoning about mechanical assembly. Artificial Intelligence, 71:371–396, 1994.

R.H. Wilson. Minimizing user queries in interactive assembly planning. IEEE Transactions on Robotics and Automation, 11 (2), April 1995.
